Robust and Practical Solution of Laplacian Equations by Approximate Elimination

We introduce a new algorithm and software for solving linear equations in symmetric diagonally dominant matrices with non-positive off-diagonal entries (SDDM matrices), including Laplacian matrices. We use pre-conditioned conjugate gradient (PCG) to solve the system of linear equations. Our preconditioner is a variant of the Approximate Cholesky factorization of Kyng and Sachdeva (FOCS 2016). Our factorization approach is simple: we eliminate matrix rows/columns one at a time and update the remaining matrix using sampling to approximate the outcome of complete Cholesky factorization. Unlike earlier approaches, our sampling always maintains a connectivity in the remaining non-zero structure. Our algorithm comes with a tuning parameter that upper bounds the number of samples made per original entry. We implement our algorithm in Julia, providing two versions, AC and AC2, that respectively use 1 and 2 samples per original entry. We compare their single-threaded performance to that of current state-of-the-art solvers Combinatorial Multigrid (CMG), BoomerAMG-preconditioned Krylov solvers from HyPre and PETSc, Lean Algebraic Multigrid (LAMG), and MATLAB's with Incomplete Cholesky Factorization (ICC). Our evaluation uses a broad class of problems, including all large SDDM matrices from the SuiteSparse collection and diverse programmatically generated instances. Our experiments suggest that our algorithm attains a level of robustness and reliability not seen before in SDDM solvers, while retaining good performance across all instances. Our code and data are public, and we provide a tutorial on how to replicate our tests. We hope that others will adopt this suite of tests as a benchmark, which we refer to as SDDM2023. Our solver code is available at: https://github.com/danspielman/Laplacians.jl/ Our benchmarking data and tutorial are available at: https://rjkyng.github.io/SDDM2023/

==> scaling-three-plots.tex <==
\subsection{Running Time Scaling with Problem Size}
\label{sec:scaling}

In this section, we summarize the running time scaling with problem size of AC and AC2 across all our experiments.

We show three different types of plots.
Our first plot type displays the total running time in seconds plotted against the number of non-zeros ($\nnz$) of the instances, both on a log scale. 
We also plot the function ${10^{-8} \nnz \log_{10}(\nnz)^3}$, which matches with the asymptotic running time scaling predicted by theory from \cite{KS16}.
We caution that we do not have a theoretical analysis that establishes such a running time for AC or AC2.
Figure~\ref{fig:ac-nnz-vs-time} shows this plot for AC, while Figure~\ref{fig:ac2-nnz-vs-time} shows this plot for AC2.

Our second plot type again shows running time in seconds \emph{measured relative to the non-zero count of the instance} plotted against non-zero count of the instances, with the x-axis on a log scale.
We also show the function $\frac{{10^{-8} \nnz \log_{10}(\nnz)^3}}{\nnz} = 10^{-8} \log_{10}(\nnz)^3$, i.e. the same running time fit as in the previous plots, but here normalized by non-zero count.
Figures~\ref{fig:ac-nnz-vs-timebynnz} and Figure~\ref{fig:ac2-nnz-vs-timebynnz} 
show these plots for AC and AC2 respectively.

Finally, we show a third plot type, where we plot time normalized by $\nnz \log_{10}(\nnz)^3$ against non-zero count, with the x-axis on a log scale.
If this was a an upper bound on the asymptotic running time, we should not see times increasing with non-zero count. 
The trend in our data across our many and diverse experiments is not clear, but at least the time does not appear to grow radically faster.
Figures~\ref{fig:ac-nnz-vs-timebynnzlog3nnz} and Figure~\ref{fig:ac2-nnz-vs-timebynnzlog3nnz} 
show these plots for AC and AC2 respectively.


\paragraph{AC running times.}
We first show the running time plots for AC as described in the previous section. 
We use a blue circle to show successful solves and a red square to show solves that failed to reach the target tolerance. 
All failed solves occurred on \emph{Sachdeva star} instances.

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac-nnz-vs-time.png}
  \caption{
  The plot shows data from all our experiments with the AC with 
  total running time in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves that reached the target tolerance are shown with a blue circle, while solves that failed to reach tolerance are shown with a red square. 
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count.
  }
  \label{fig:ac-nnz-vs-time}
\end{figure}

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac-nnz-vs-timebynnz.png}
  \caption{
  The plot shows data from all our experiments with the AC with 
  total running time \emph{per non-zero} in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves that reached the target tolerance are shown with a blue circle, while solves that failed to reach tolerance are shown with a red square. 
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count, and the same normalization is used as for the data (i.e. dividing by $\nnz$).
  }
  \label{fig:ac-nnz-vs-timebynnz}
\end{figure}

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac-nnz-vs-timebynnzlog3nnz.png}
  \caption{
  The plot shows data from all our experiments with the AC with 
  total running time \emph{divided by $\nnz \log_{10}(\nnz)^3$} in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves are shown with a blue circle. All solves reached the target tolerance.
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count, and the same normalization is used as for the data (i.e. dividing by $\nnz \log_{10}(\nnz)^3$).
  }
  \label{fig:ac-nnz-vs-timebynnzlog3nnz}
\end{figure}

\paragraph{AC2 running times.} We now show running time plots for AC2 as described earlier. 
We use a blue circle to show successful solves. For AC2, all solves reached the tolerance (i.e. $1e-8$ relative residual error).

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac2-nnz-vs-time.png}
  \caption{
  The plot shows data from all our experiments with the AC2 with 
  total running time in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves are shown with a blue circle. All solves reached the target tolerance.
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count.
  }
  \label{fig:ac2-nnz-vs-time}
\end{figure}

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac2-nnz-vs-timebynnz.png}
  \caption{
  The plot shows data from all our experiments with the AC2 with 
  total running time \emph{per non-zero} in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves are shown with a blue circle. All solves reached the target tolerance.
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count, and the same normalization is used as for the data (i.e. dividing by $\nnz$).
  }
  \label{fig:ac2-nnz-vs-timebynnz}
\end{figure}

\begin{figure}[H]
  \centering
\includegraphics[width=0.7\textwidth]{fig/ac2-nnz-vs-timebynnzlog3nnz.png}
  \caption{
  The plot shows data from all our experiments with the AC2 with 
  total running time \emph{divided by $\nnz \log_{10}(\nnz)^3$} in seconds on the y-axis plotted against 
  the number-of-non-zeros of the instance on the x-axis.
  Solves that reached the target tolerance are shown with a blue circle, while solves that failed to reach tolerance are shown with a red square. 
  An orange line shows the function $\nnz \log_{10}(\nnz)^3$ (seconds) where $\nnz$ is the non-zero count, and the same normalization is used as for the data (i.e. dividing by $\nnz \log_{10}(\nnz)^3$).
  }
  \label{fig:ac2-nnz-vs-timebynnzlog3nnz}
\end{figure}




==> scrap.tex <==








In the implementation {\AC}, we use a preconditioner based on the
approximate Cholesky Factorization computed by
\textsc{ApproximateEdgewiseCholesky}
(Algorithm~\ref{alg:ApproximateEdgewiseCholesky}).
This algorithm uses the clique sampling
$\textsc{CliqueTreeSample}$ for elimination, and outputs the
approximate factorization in a row operation representation.
To apply the preconditioner, we use forward and backward substitution,
combined with Equation~\eqref{eq:pinvproduct}.

In the implementation {\ACSM}, we use a preconditioner based on the
approximate Cholesky Factorization computed by
\textsc{ApproximateEdgewiseCholesky}
(Algorithm~\ref{alg:ApproximateEdgewiseCholesky}),
but with the clique
sampling algorithm \textsc{ApproximateEdgewiseCholesky} replaced by
\textsc{CliqueTreeSampleMultiEdgeMerge} (Algorithm \ref{alg:CliqueTreeSampleMultiEdgeMerge}).
Again, to apply the preconditioner, we use forward and backward substitution,
combined with Equation~\eqref{eq:pinvproduct}.

Details of our elimination ordering choices are described in Section~\ref{sec:elimorder}.





Since $\textsc{CliqueTreeSample}$ outputs exactly one edge sample per
neighbor of the vertex being eliminated, we can immediately deduce the
following corollary.
\begin{corollary}
  \label{cor:ourapxcholfillin}
  When $\textsc{ApproximateCholesky}$
  (Algorithm~\ref{alg:GeneralApproximateCholeskyFactorizationColwise})
 is used with the sampling routine $\textsc{CliqueSample}$ and with a
 random elimination ordering, then the total expected number of
 non-zeros in the output $\matlow$ is bounded
  by $O(|E|\log|E|)$, where $|E|$ is the number of edges in the graph
  of the input Laplacian.
\end{corollary}
























\resizebox{\textwidth}{!}{%
\begin{tabular}{
      |c
    | S[table-format=1.2] S[table-format=2.2]  
    | S[table-format=1.3] S[table-format=1.3] S[table-format=1.2]  S[table-format=1.2]
    |
}
\hline
    \multirow{3}{*}{Instance family}
&  {AC}   & {{\ACSM}}     
& {CMG}  &  {HyPre}   &  {PETSc}        & {ICC}    
    \\
\cline{2-7} 
    &
    &{ $t_{\text{total}} / \nnz $ }               
    &
    &{ $t_{\text{total}} / \nnz $ }
    &
    &
    \\
\cline{2-7} 
& {$(\mu s)$} & {$(\mu s)$} 
& {$(\mu s)$}  &  {$(\mu s)$}  & {$(\mu s)$}  & {$(\mu s)$}\\ \hline %
{SuiteSparse Matrix Collection}&1.5e+04&1.51e+04&Inf&Inf&Inf&Inf\\
{Unweighted chimeras}&4.05&7.28&Inf&Inf&Inf&Inf\\
{Weighted chimeras}&5.21&5.02&Inf&Inf&N/A&Inf\\
{Unweighted SDDM chimeras}&3.6&5.54&Inf&Inf&Inf&Inf\\
{Weighted SDDM chimeras}&4.97&4.84&Inf&Inf&N/A&Inf\\
{Maximum flow IPMs}&1.4&2.58&\textcolor{red}{1.9}&\textcolor{blue}{5.04}&N/A&Inf\\
{Sachdeva stars}&\textcolor{red}{4.89}&1.04&0.868&\textcolor{red}{3.52}&\textcolor{red}{7.22}&Inf\\
{SPE benchmark}&1.78&2.3&0.511&0.648&2.58&4.29\\
{Uniform coefficient Poisson grid}&1.66&2.58&0.624&0.587&2.62&2.22\\
{High contrast coefficient Poisson grid}&3.06&4.1&0.572&0.752&3.85&4.76\\
{Anisotropic coef. Poisson grid, variable discretization}&1.69&2.61&0.659&0.614&2.6&1.92\\
{Anisotropic coef. Poisson grid, variable weight}&2.03&2.7&0.674&0.772&4.92&2.44\\
    \hline
  \end{tabular}
} %




\begin{center}
    \small
\begin{tabularx}{\textwidth}{ | X | }
\hline
 \textcolor{blue}{blue: residual error exceeded tolerance by a factor ...} \\  
 \textcolor{red}{red: residual error exceeded tolerance by a factor ...} \\  
 N/A: Experiment with PETSc omitted as the solver crashed too often.  \\
\hline
\end{tabularx}
\end{center}








\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{
      |c
    | S[table-format=1.2] S[table-format=2.2]  
    | S[table-format=1.3] S[table-format=1.3] S[table-format=1.2]  S[table-format=1.2]
    |
}
\hline
    \multirow{3}{*}{Instance family}
&  {AC}   & {{\ACSM}}     
& {CMG}  &  {HyPre}   &  {PETSc}        & {ICC}    
    \\
\cline{2-7} 
    &
    &{ $t_{\text{total}} / \nnz $ }               
    &
    &{ $t_{\text{total}} / \nnz $ }
    &
    &
    \\
\cline{2-7} 
& {$(\mu s)$} & {$(\mu s)$} 
& {$(\mu s)$}  &  {$(\mu s)$}  & {$(\mu s)$}  & {$(\mu s)$}\\ \hline %
{SuiteSparse Matrix Collection}&1.5e+04&1.51e+04&Inf&Inf&Inf&Inf\\
{Unweighted chimeras}&4.05&7.28&Inf&Inf&Inf&Inf\\
{Weighted chimeras}&5.21&5.02&Inf&Inf&N/A&Inf\\
{Unweighted SDDM chimeras}&3.6&5.54&Inf&Inf&Inf&Inf\\
{Weighted SDDM chimeras}&4.97&4.84&Inf&Inf&N/A&Inf\\
{Maximum flow IPMs}&1.4&2.58&\textcolor{red}{1.9}\tnote{**}&\textcolor{blue}{5.04}\tnote{*}&N/A&Inf\\
{Sachdeva stars}&\textcolor{red}{4.89}&1.04&0.868&\textcolor{red}{3.52}&\textcolor{red}{7.22}&Inf\\
{SPE benchmark}&1.78&2.3&0.511&0.648&2.58&4.29\\
{Uniform coefficient Poisson grid}&1.66&2.58&0.624&0.587&2.62&2.22\\
{High contrast coefficient Poisson grid}&3.06&4.1&0.572&0.752&3.85&4.76\\
{Anisotropic coef. Poisson grid, variable discretization}&1.69&2.61&0.659&0.614&2.6&1.92\\
{Anisotropic coef. Poisson grid, variable weight}&2.03&2.7&0.674&0.772&4.92&2.44\\
    \hline
  \end{tabular}
\begin{tablenotes}
\footnotesize
\item[*] residual error exceeded tolerance by a factor ...
\item[**] residual error exceeded tolerance by a factor ...
\item[] \hspace{-1em} Inf: Solver crashed or returned a solution with relative residual error 1 (trivial solution).
\item[] \hspace{-1em} N/A: Experiment omitted as the solver crashed too often with (only occurred for PETSc).
\end{tablenotes}
\end{threeparttable}
} %


==> summarytable-residuals.tex <==
\resizebox{\textwidth}{!}{%
  \begin{tabular}{
      |c
    |S[table-format=1.3e1] S[table-format=1.3]
    | S[table-format=1.3e-1]S[table-format=2.3e1] S[table-format=3.5e1]  S[table-format=1.3e1]
    |
}
\hline
    \multirow{3}{*}{Instance family}
    &  {AC}   & {{\ACSM}}     
    & {CMG}  &  {HyPre}   &  {PETSc}         & {ICC}    
    \\
\cline{2-7} 
    &
    &{ res. err. }               
    &
    &{ res. err. }
    &
    &
    \\
\cline{2-7} 
& {$(10^{-8})$} & {$(10^{-8})$} 
& {$(10^{-8})$} & {$(10^{-8})$} & {$(10^{-8})$} & {$(10^{-8})$} \\ \hline %
    {Uniform coefficient Poisson grid}&
    0.878&0.843&0.982&0.206&0.00518&0.974\\
    {High contrast coefficient Poisson grid}&
    0.986&0.98&0.952&0.98&0.00142&0.994\\
    {Anisotropic coef. Poisson grid, variable discretization}&
    0.952&0.987&0.982&0.205&0.116&0.999\\
    {Anisotropic coef. Poisson grid, variable weight}&
    0.988&0.792&0.972&0.618&0.0704&0.995\\
    {Unweighted chimeras}&
    0.992&0.997&Inf&Inf&Inf&1e+08\\
    {Weighted chimeras} &
    0.998&0.996&Inf&Inf&Inf&1e+08\\
    {Unweighted SDDM chimeras}&
    0.989&0.495&Inf&Inf&Inf&1e+08\\
    {Weighted SDDM chimeras} &
    0.989&0.989&Inf&Inf&Inf&1e+08\\
    {Sachdeva Stars} &
    4.1e+05&0.965&3.85e-06&2.71e+06&2.76e+04&1e+08\\
    {SPE benchmark} &
    0.617&0.623&0.884&0.384&0.00939&0.999\\
    {SuiteSparse Matrix Collection} &
    0.999&0.884&Inf&Inf&Inf&1e+08\\
    {IPM} &
    0.844&0.998&1.35e+04&0.858&4.46&Inf\\
    \hline
  \end{tabular}
} %

